Estimating the parameters of ocean wave spectra

Wind-generated waves are often treated as stochastic processes. There is particular interest in their spectral density functions, which are often expressed in some parametric form. Such spectral density functions are used as inputs when modelling structural response or other engineering concerns. Therefore, accurate and precise recovery of the parameters of such a form, from observed wave records, is important. Current techniques are known to struggle with recovering certain parameters, especially the peak enhancement factor and spectral tail decay. We introduce an approach from the statistical literature, known as the de-biased Whittle likelihood, and address some practical concerns regarding its implementation in the context of wind-generated waves. We demonstrate, through numerical simulation, that the de-biased Whittle likelihood outperforms current techniques, such as least squares fitting, both in terms of accuracy and precision of the recovered parameters. We also provide a method for estimating the uncertainty of parameter estimates. We perform an example analysis on a data-set recorded off the coast of New Zealand, to illustrate some of the extra practical concerns that arise when estimating the parameters of spectra from observed data.

==> Estimating the parameters of ocean wave spectra - final/extra_commands.tex <==

% \usepackage{amsthm} % Needed to typeset theorem environments.
%\usepackage{MnSymbol}
\newcommand{\Dft}[2]{D_{#1,#2}}%d_N(\omega\mid X_\Delta)
\newcommand{\periodogram}[2]{I}%{I_{#1,#2}}
\newcommand{\sumXt}[2]{\sum^{#1}_{t=1}X_{t#2}\exp\{-it#2\omega\}}
\newcommand{\sumOmega}[3]{\sum_{\omega\in\Omega_#1}#3\exp\{it#2\omega\}}
\newcommand{\sumDo}[2]{\sumOmega{#1}{#2}{\Dft{#1}{#2}(\omega)}}
\newcommand{\mysqrt}[1]{\left(#1\right)^{\frac{1}{2}}}
\newcommand{\Exponential}[1]{\text{Exponential}\left(#1\right)}
\newcommand{\cNorm}[2]{\mathcal{CN}\left(#1,#2\right)}
\newcommand{\Norm}[2]{\mathcal{N}\left(#1,#2\right)}
\newcommand{\acf}{c}
%%

% Commands for special set of numbers.

\newcommand{\varhat}[1]{\, {\rm \hat{var}}\left( #1 \right) }
\newcommand{\covhat}[1]{\, {\rm \hat{cov}}\left( #1 \right) }


% commands for model
\newcommand{\expbit}{\exp\left \{-\frac{r}{s}\left(\frac{\omega}{\omega_p}\right)^{-s}\right \}}
% \newcommand{\parbit}{\omega,\alpha,\omega_p,\gamma,r}
% \newcommand{\minusparbit}{-\omega,\alpha,\omega_p,\gamma,r}
\newcommand{\parbit}{\omega\mid\theta}
\newcommand{\minusparbit}{-\omega\mid\theta}
\newcommand{\dbit}{\delta(\parbit)}
\newcommand{\sigbit}{\sigma(\parbit)}
\newcommand{\fbit}{f_G(\parbit)}
\newcommand{\gbit}{g(\parbit)}
\newcommand{\Sbit}{S_G(\parbit)}
\newcommand{\pard}[1]{\frac{\partial}{\partial #1}}
\newcommand{\negderiv}[1]{\pard{#1}\fbit&=\pard{#1}f_G(\minusparbit)}

% commands that need notational checking
\newcommand{\XN}{\bX_{\Delta,N}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bx}{\boldsymbol{x}}

% Theorem definitions/
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{theorem}[lemma]{Theorem}
% \newtheorem{proposition}[lemma]{Proposition}
% \newtheorem{corollary}[lemma]{Corollary}


%% matlab logo
\newcommand{\matlab}{MATLAB }

==> Estimating the parameters of ocean wave spectra - final/preamble.tex <==
%---------------------------------------------------------%
%------------------ Document Preamble --------------------%
%---------------------------------------------------------%

%-------------------------------------------%
%---- First load the necessary packages ----%
%-------------------------------------------%

\usepackage{graphicx} % For including graphics (via \includegraphics).
\usepackage{amsmath}  % Improves typographic quality of mathematical output.
\usepackage{amsfonts} % For mathematical fonts.
\usepackage{import} %for nice pics
% Package for no indentation and to include a line between paragraphs.
\usepackage[parfill]{parskip}

% Set the layout of the document.
%\usepackage[margin=2.5cm,scale=1,vmarginratio={1:2},heightrounded]{geometry}
\usepackage[margin=2.5cm]{geometry}
%\usepackage{fullpage}
\usepackage{amsthm} % Needed to typeset theorem environments.
\usepackage[affil-it]{authblk} % Needed for author and affiliation.
\usepackage{amsopn} % Allows the declaration of new mathematical operators.
\usepackage{amssymb} % Extended set of mathematical symbols.
\usepackage{mathrsfs} % Raph Smith's mathematical script font.
\usepackage{booktabs} % Improves the typographical quality of tables.
\usepackage{natbib} % Citations and bibliography.
\usepackage{tikz} % Extends the figure generation capabilities of LaTeX.
\usepackage{algorithm} % Necessary for including algorithmic structures.
\usepackage{float} % Allows the creation of own floating environments.
\usepackage{caption} % Allows the customisation of captions.
\usepackage{abstract} % For including abstracts in documents.
\usepackage{listings} % For the inclusion of source code.
\usepackage{color} % Used for colour commands.
\usepackage{enumerate} % Used for nicer numberings
\usepackage{fancyvrb} % Nicer verbatim
\usepackage{float}
\usepackage{subcaption}

% Automatic inclusion of hyperlinks with back references.
\usepackage[]{hyperref} %pagebackref

%-------------------------------------------%

% Making a float for an algorithm.
\newfloat{algorithm}{t}{lop}
\renewcommand{\thealgorithm}{\arabic{section}.\arabic{algorithm}} 

% Numbers equations by section.
% \numberwithin{equation}{section}

% Set biliography style.
\bibliographystyle{apalike}

% Commands for special set of numbers.
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\EE}[1]{\mathbb{E} \left[ #1 \right]}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\e}[1]{{\textrm{e}}^{#1}}
% Commands for useful operators.
\newcommand{\di}{\text{diag}}
\newcommand{\de}{\mathrm{d}}
\newcommand{\si}{\Sigma}
\newcommand{\del}{\Delta}
\newcommand{\cov}[1]{\, {\rm cov}\left( #1 \right) }
\newcommand{\var}[1]{\, {\rm var}\left( #1 \right) }
\newcommand{\cum}[1]{\, {\rm cum}\left( #1 \right) }
\newcommand{\toas}{\xrightarrow{\text{a.s.}}}
\newcommand{\todis}{\xrightarrow{\text{d}}}
\newcommand{\supp}{\text{supp}}
\newcommand{\abs}{\text{abs}}
\newcommand{\doubint}{\!\int\!\!\!\int}
\DeclareMathOperator*{\argmin}{argmin} % no space, limits underneath in displays
\DeclareMathOperator*{\argmax}{argmax} % no space, limits underneath in displays
% Command for text within a math sub/super-script.
\newcommand{\stext}[1]{\text{\scriptsize{#1}}}

% Theorem definitions/
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{corollary}[lemma]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\theoremstyle{remark}
\newtheorem{remark}{Remark}[section]
\newtheorem{example}[remark]{Example}

% My own theorem environment for task 2 exercise 6
\theoremstyle{theorem}
\newtheorem{theory}[lemma]{Theory}

% An environment for centre aligning equations which extend past the text width.
\newenvironment{longeq}
 {\begin{displaymath}\begin{lrbox}{\overlongequation}$\displaystyle}
 {$\end{lrbox}\makebox[0pt]{\usebox{\overlongequation}}\end{displaymath}}

% Listings options.

\lstset{ %
basicstyle=\footnotesize,       % the size of the fonts that are used for the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}
%%% tikz stuff
%% In order to be able to put arrowheads in the middle of directed edges, we need an extra library.
\usetikzlibrary{decorations.markings}
\usetikzlibrary{graphs,graphs.standard,quotes}

